Graph-based Molecular Representation Learning

Molecular representation learning (MRL) is a key step to build the connection between machine learning and chemical science. In particular, it encodes molecules as numerical vectors preserving the molecular structures and features, on top of which the downstream tasks (e.g., property prediction) can be performed. Recently, MRL has achieved considerable progress, especially in methods based on deep molecular graph learning. In this survey, we systematically review these graph-based molecular representation techniques, especially the methods incorporating chemical domain knowledge. Specifically, we first introduce the features of 2D and 3D molecular graphs. Then we summarize and categorize MRL methods into three groups based on their input. Furthermore, we discuss some typical chemical applications supported by MRL. To facilitate studies in this fast-developing area, we also list the benchmarks and commonly used datasets in the paper. Finally, we share our thoughts on future research directions.

==> resources/all_papers_topconferences.tex <==
\begin{table*}
\vspace{-0.15in}
\caption{Taxonomy and Representative Publications of Molecule Representation Learning.}
\vspace{-0.15in}
\label{tab:main_algorithm}
\begin{center}
\scale[0.75]{{\begin{tabular}{l|l|l|p{6cm}}
\toprule
\textbf{Paper} & \textbf{Task} & \textbf{Dataset} &\textbf{summary} \\ 
\midrule
\cite{boomsma2017spherical} & predict protein change-of-stability & / & conducting convolutions on the sphere to learn molecular image datasets\\
WLDN~\cite{jin2017predicting}&Reaction Prediction &USPTO,USPTO-15K &Template-free method to prediction reaction center then enumerate candidate products. Use WLN to score final product\\
MPNN\cite{gilmer2017neural} &Property prediction &QM9 &General framework, message passing phase and readout phase to learn\\
ChemNet\cite{goh2018using} &Property prediction &MoleculeNet & Rule-based knowledge for pretraining image molecules\\
AttSemiGAE\cite{ma2018drug} &adverse drug-drug interaction(0/1)&DDi, Lable side effect &multiview GAE and attentive mechanism to corresponding tasks and features for better interpretability.\\
E2E\cite{gao2018interpretable} &drug target interaction(drug discovery 0/1) &BindingDB &End-to-end DTI, GraphCNN encode drug, lstm encode protein and provide biologycal interpretation using two-way attentio mechnism\\
CDN\cite{harel2018accelerating} &drug discovery(generate) &ZINC and DrugBank &VAE to encoder and add diversity layer to extend generation process then decoder to generate new drugs\\
JT-VAE\cite{jin2018junction} &molecular generation &ZINC &generate molecular graph in two phases by exploiting valid subgraphs as component. generate junction tree then assembled into a molecular graph\\
MGCN\cite{lu2019molecular} &Property prediction &QM9, ANI-1 &multi-level hierarchical GCN extract features from the conformation and spatial information by multilevel interactions. \\
NEVAE\cite{samanta2020nevae} &molecular generation &ZINC, QM9 &VAE based on GNN for molecular nodes and edges,decoder is able to provide spatial coordinates of the atoms of molecules. greater stability and maximize the value of interest property \\
N-Gram Graph\cite{liu2019n} &molecular property prediction &Qm9, MoleculeNet &N-gram graph, embeds the vertexes in the graph and essembling the vertext embeddings in short walks in graph \\
MoleculeChef\cite{bradshaw2019model} &Synthesizable molecular generation &USPTO &GGNN encode reactants VAE generates reactants then use molecular transformer to prediction products\\
VJTNN\cite{jin2018learning} &molecular optimization (generation?) &Drug likeness, DRD2 &generate junction tree then use MPNN encode tree and tree-decoder and graph -decoder generate graph \\
MHG-VAE\cite{kajino2019molecular} &moleclar optimization &ZINC &transfer graph to hypergraph and using MHG to generate sparse sequence, then use GVAE to generate molecule \\
CASTER\cite{huang2020caster} &adverse drug drug interaction &DDI, BIOSNAP &algorithm to collect substructures of two drugs then use sequential encoder and decoder. add dictionary module to explain the prediction.\\
CIGIN\cite{pathak2020chemically} &solvation free energies &Minnesota Solvation &MPNN solute and solvent, then calculate interaction features, interpretable\\
CORE\cite{fu2020core} &molecular optimization &ZINC &MPN encoder graph and scaffoling tree then tree decoder to decide whether to copy a substurcture from the input molecule or smaple a novel substructure from entire space. Graph decoder to sample.\\
CMPNN\cite{songcommunicative} &property prediction &MoleculeNet &Add communication function to strengthen message interaction with nodes and edges \\
KGNN\cite{lin2020kgnn} &drug-drug interaction &DrugBank, KEGG-drug &Build knowledge graph learn drugs embedding according to KG then prediction interaction\\
ASGN\cite{hao2020asgn} &property prediction &QM9, OPV &teacher student framework, semi-supervised pretrain teacher, active learning to select informative data finetune student.\\
@@MNCE-RL\cite{xu2020reinforced} &Molecular optimization &LogP, QED &neighborhood controlled embedding grammars and efficient reinforcement learning algorithm to generate valid moelcules\\ 
@@GEGL\cite{ahn2020guiding} &molecular optimization & &expert-guided learning, expert policy and apprentive policy, using max-reward priority queues to push model generate best molecules LSTM as encoder\\
***GROVER\cite{rong2020self} &property prediction &ZINC15, Chembl pretrain, MoleculeNet &Gtransformer to learn graph embedding, pretrain tasks like contextural property prediction(predict masked atom, bond and substructure) and predict graph-level motif\\
RetroXpert\cite{yan2020retroxpert} &retrosynthesis prediction &USPTO, USPTO-50K, USPTO-full &Use Edge-enhanced GAT(EGAT) to predict reaction center and split the target molecule according to center to obtain synthons, then use reactant generation network to use target molecule and synthons to generate reactants.(seq2seq)\\
CogMol\cite{chenthamarakshan2020cogmol} &drug design for covid & &deep generative model to generate good molecules for COVID\\
GraphCL\cite{you2020graph} &property prediction &NCI1, PROTEINS &Use node dropping, edge perturbation, attribute masking to do data augmentation to do contrastive learning\\
DimeNet\cite{klicpera2019directional} &property prediction, molecular dynamics &QM9, MD17 &directional GNN based on distance between atoms and the angle between directions, distance represented by spherical Bessel functions, angles represented by 2D spherical Fourier-Bessel basis\\
GraphAF\cite{shi2020graphaf} &molecular generation &ZINC &flow-based autoregressive model, dynamically generates nodes and edges, define feedforward NN to compute the data likelihood in parallel\\
RationaleRL\cite{jin2020multi} &drug discovery &GNK3\beta,JNK3 &generate retionales(key property realted structure) from molecules, then expand rationales into full molecule using MPN VAE, supervised\\
***HierVAE\cite{jin2020hierarchical} &Molecular generation &LogP, QED, DRD2 &encode and decode to generate graph in a hierarchical way, motif layer predict motif, attachment layer predict connect method between motif, atom layer predict how atom connected.\\
GNN-FiLM\cite{brockschmidt2020gnn} &property predicton &QM9 &the representation of the target node of an edge is used to compute a transformation that can be applied to all incoming messages, allowing featurewise modulation of the passed information\\
MIMOSA\cite{fu2020mimosa} &molecule generation &ZINC &pretrain GNN then use prediction adn emplys operations(add, replace, delete) to generate molecules and associated weights which have multiple contraints.\\
MolGrow\cite{kuznetsov2021molgrow} &molecular generation &QM9, ZINC &hierarchical normalizing flow model for generating molecular graph.\\
SafeDrug\cite{yangsafedrug} &drug-drug interaction &MIMIC-III &global MPNN and local bipartitle learning module to encode connectivity and functionality of drug molecuels also RNN encode patient representations.\\
@@CSGNN\cite{zhao2021csgnn} &molecular interactions &a lot &Molecular interaction network, build mix-hop GNN to model and design contrastive learning model to make graph different from corrupted graph\\
MDNN\cite{lyumdnn} &drug-drug-interaction &DDIMDL, DrugBank &Two path way, drug knowledge graph and heterogeneous features to learn molecular representations to predict\\
***MoCL\cite{sun2021mocl} &property prediction &MoleculeNet &maximize mutual information: two augmented view and two similar graph: local-level domain knowledge, add replace functional group and add/drop general carbon to contrastive methods, for global-level, calculate graph similarity.\\
UGMMT\cite{barshatski2021unpaired} &molecular optimization &DRD2, QED &(smiles) unsupervised end-to-end generative model and a unique double-cycle training scheme for molecule translation preserving molecule similarity using molecular fp utilization, without the need of a large paired dataset\\
@@BDKANN\cite{snow2021interpretable} &drug disease &GDSCV2, CTRPv2 &domain and biological knowledge based methods \\
GEOMOL\cite{ganea2021geomol} &Molecular 3D conformer ensembles &GEOM-Q9, GEOM-DRUGS &Leveraging the power of message passing neural networks (MPNNs) to capture local and global graph information, we predict local atomic 3D structures and torsion angles, avoiding unnecessary over-parameterization of the geometric degrees of freedom (e.g. one angle per non-terminal bond)\\
***MGSSL\cite{zhang2021motif} &property prediction & &generate motifs, use GNN to generate motif tree and prediction motif label to pretrain GNN, also mask bonds, atoms to pretrain GNN on molecular graph. \\
DGSM\cite{luo2021predicting} &3D conformation &GEOM-Q9, GEOM-Drugs &dynamically construct graph structures with non-bonded edges between atom pairs within a distance based on the current spatial proximity, dynamic graph score matching algorithm, where graph structures are also dynamically determined during training depending on added perturbations\\
***PhysChem\cite{yang2021deep} &property prediction &MoleculeNet &Physnet and chemnet, PhysNet is a neural physical engine that learns molecular conforma- tions through simulating molecular dynamics with parameterized forces; ChemNet implements geometry-aware deep message-passing to learn chemical / biomedical properties of molecules\\
***PAR\cite{wang2021property} &property prediction &MoleculeNet &property aware embedding function to transform embeeding to target property, and build molecular graph\\
***GemNet\cite{klicpera2021gemnet} &molecular interaction &COLL, MD17, OC20 &propose edge-based two-hop message passing scheme geometric message passing and propose multiple structural enhancements to improve the practical performance of this formalism\\
FREED\cite{yang2021hit} &molecular generation &DUD-E, ChEMBL &reinforcement learning model with a prioritized experience replay method to defines priority and generate molecules based on molecular fragments\\
***directional MPNN\cite{klicpera2021directional} &property prediction &ZINC, QM9 &Use synthetic coordinates to calculate bounds of pairwise distances, calculate bounds of distances and angles then use directional MPNN to learn graph\\
MARS\cite{xie2020mars} &drug discovery &ChEMBL &employs Markov chian Monte Carlo sampling molecules and use GNN to generate candidate \\
INFOGRAPH\cite{sun2019infograph} &property prediction &QM9 &maximize the mutual information between the representations of entire graphs and the representations of substructures of different granularity(patch)\\
PreGNN\cite{hu2019strategies}&property prediction &MoleculeNet &contextual prediction, attribute masking pretraining strategies  \\
GraphDF\cite{luo2021graphdf} &molecular generation &ZINC, QM9 &generates molecular graphs by sequentially sampling discrete latent variables and mapping them to new nodes and edges via invertible modulo shift transforms\\
PAINN\cite{schutt2021equivariant} &Tensorial properties, molecular spectra &QM9 &polarizable atom interaction neural network. extend the message passing formulation to rotationally equivariant representations.\\
GCNN\cite{henderson2021improving} & property prediction & &add batch representation orthonormalization and Gini regularization to improve molecular GNN explainability\\
ConfGF\cite{shi2021learning} & molecular conformation generation & &ConfGF by directly esti- mating the gradient fields of the log density of atomic coordinates. The estimated gradient fields allow directly generating stable conformations via Langevin dynamics. \\
ConfVAE\cite{xu2021end} &molecular conformation generation &GEOM-Drugs &conditional VAE, gnn as encoder, 3D sturctures are generated by solving a principled bilevel optimization program\\
NERF\cite{bi2021non}&reaction prediction&USPTO-15k &conditional VAE as encoder, decoder estimate flow of electron pairs to reflect the changes of edges \\
***KCL\cite{fang2022molecular} &property prediction &MoleculeNet &Using chemical element KG to add associations between atoms that have comment attributes but not directly connected. heterogeneous message passing to learn representation. contrastive loss\\
spreadGNN\cite{he2022fedcv}&property prediction &MoleculeNet &serverless multi-task federated learning forGNN \\
***GeomMPNN\cite{li2022geomgcl} &property prediction &MoleculeNet &deterministic mapping obtain 2D graph, Stochastic mapping obtain 3D graph. Geometric embedding and message passing two views and using contrastive loss to self-supervised\\
GEODIFF\cite{xu2022geodiff} &molecular conformation generation &GEOM-QM9, GEOM-Drugs &Markov chains evolving with equivariant Markov kernels can induce an invariant distribution by design, and further propose building blocks for the Markov kernels to preserve the desirable equivariance property\\
DEG\cite{guo2022dataefficient} &molecular generation & &a learnable graph grammar that generates molecules from a sequence of production rules, spanning forest build by all input graphs\\
STGG\cite{ahn2022spanning} &molecular generation &QM9, ZINC250K, MOSES & Transformer architecture with tree-based relative positional encodings for realizing the tree construction procedure\\
TorchMD-NET\cite{tholke2022equivariant} &property prediction &QM9, MD17, ANI-1 &novel equivariant transformer architecture. interatomic distances modified transformer attention mechanism\\
MoLeR\cite{maziarz2022learning} &molecular generation & &GNN supports scaffolds as initial seed of generation process based on motifs\\
MolR\cite{wang2022chemicalreactionaware}&property prediction, reaction prediction & Molecule Net, USPTO & embeddings equivalence between reactants and products\\
ChIRo\cite{adams2022learning} &property prediction & &2D MPNN and two feed forward networks to encode 3D bond distances and bond angles encode chirality\\
DST\cite{fu2022differentiable} &molecular optimization & &Differentiable scaffolding tree, enables a gradient-based optimization on a chemical graph structure by back-propagating the derivatives from the target properties through a graph neural network\\
***GRAPHMVP\cite{liu2022pretraining} &property prediction &GEOM &2d and 3d graph embeding，using SSL constructive and generative tasks to pretrain the model\\
G-SphereNet\cite{luo2022an} &molecular geometry generation & &flow model to generate 3D molecular geometry generation\\
SphereNet\cite{liu2022spherical} & & &propose the spherical message passing (SMP) as a novel and powerful scheme for 3D molecular learning\\
GNS+noise nodes\cite{godwin2022simple} &property prediction &OGB &add noise node to avoid over smoothing problems\\
DGAPNs\cite{wu2022spatial} &drug discovery &MCULE &reinforcement learning architecture to construct a fragment-based action space and propose a GAT to encode node, bonds and spatial structures\\
\bottomrule
\end{tabular}}}
\end{center}
\end{table*}


==> tables/Papers_overview_lateset.tex <==
\begin{table*}
% \vspace{-0.15in}
\caption{Taxonomy and Representative Publications of Molecule Representation Learning.}
\vspace{-0.15in}
\label{tab:main_algorithm}
\begin{center}
\scale[0.6]{{\begin{tabular}{l|l|l|l|l|l}
\toprule
\textbf{Algorithm} & \textbf{Task} & \textbf{Encoder} &\textbf{Venue} &\textbf{Reference} &\textbf{Link}\\ 
\midrule \midrule
\multicolumn{6}{c}{Graph-based Learning} \\
\midrule
MPNN & Property prediction & MPNN & IMLR'17
&\cite{gilmer2017neural} & / \\
DimeNet & Property prediction + Molecular dynamics & MPNN & ICLR'19 & \cite{klicpera2019directional} &\hyperlink{https://github.com/klicperajo/dimenet}{[Code Link]} \\
GNN-FiLM & Property prediction & MPNN & ICML'20 & \cite{brockschmidt2020gnn} &\hyperlink{https://github.com/microsoft/tf-gnn-samples}{[Code Link]}\\
GROVER &property prediction &GAT &NeurIPS'20 &\cite{rong2020self} &\url{https://github.com/tencent-ailab/grover}\\
Pre-GNN & Property prediction & GIN & ICLR'20 &\cite{Hu2020Strategies} &\url{https://github.com/snap-stanford/pretrain-gnns/}\\
INFOGRAPH &property prediction &GNN &ICLR'20 &\cite{sun2020infograph}  &\url{https://github.com/fanyun-sun/InfoGraph}\\
GraphCL &property prediction &GNN &NeurIPS'20 &\cite{you2020graph} &\url{https://github.com/Shen-Lab/GraphCL}\\
PAR & Property prediction & GIN & NeurIPS'21 &\cite{wang2021property} & /\\
Meta-MGNN & Property prediction & GIN & WWW'21 & \cite{guo2021few} &\url{https://github.com/zhichunguo/Meta-MGNN} \\
GCNN& property prediction &GNN &ICML'21 &\cite{henderson2021improving} &\url{https://github.com/bayer-science-for- a-better-life/graph-attribution.} \\
MoCL & Property prediction & GIN & KDD'21 &\cite{sun2021mocl} &\url{https://github.com/illidanlab/MoCL-DK}\\
MGSSL & Property prediction & GIN & NeurIPS'21 &\cite{zhang2021motif} &\url{https://github.com/zaixizhang/MGSSL}\\
PhysChem & Property prediction & LSTM & NeurIPS'21 &\cite{yang2021deep} & /\\
PAR & Property prediction & GIN Pre-GNN & NeurIPS'21 &\cite{wang2021property} & /\\
MolR & Property prediction + Reaction prediction& GNN & ICLR'22 & \cite{wang2021chemical} & \url{ https://github.com/hwwang55/MolR}\\
KCL &property prediction &MPNN &AAAI'22 &\cite{fang2022molecular} &\url{https://github.com/ZJU-Fangyin/KCL}\\
GeomGCL &property prediction &MPNN &AAAI'22 &\cite{li2022geomgcl} & /\\
GRAPHMVP &property prediction &3D GNN &ICLR'22 &\cite{liu2022pretraining}  &\url{https://github.com/chao1224/GraphMVP}\\
SphereNet &Property Prediction + dynamics simulation &spherical message passing &ICLR'22 &\cite{liu2022spherical} &\url{https://github.com/Open-Catalyst-Project/ocp}\\
\midrule
WLDN & Reacton prediction & Weisfeiler-Lehman isomorphism test & NeurIPS'17 &\cite{jin2017predicting} &\url{https://github.com/wengong-jin/nips17-rexgen} \\
GTPN & Reaction prediction & MPNN & KDD'19 & \cite{do2019graph} & / \\
WLDN++ & Reaction prediction & GCN & Chemical Science' 19 & \cite{coley2019graph} & \url{https://github.com/connorcoley/rexgen_direct}\\
\midrule
JT-VAE & Molecule generation & MPNN & ICLR'18 &\cite{jin2018junction} &\url{https://github.com/wengong-jin/icml18-jtnn} \\
MoleculeChef &molecular generation &GGNN & NeurIPS'19 &\cite{bradshaw2019model} &\url{https://github.com/ john-bradshaw/molecule-chef}\\
GraphAF & Molecular generation & R-GCN & ICLR'20 &\cite{shi2020graphaf} &\url{https://github.com/DeepGraphLearning/GraphAF}\\
HierVAE & Molecular generation & MPN & PMLR'20 &\cite{jin2020hierarchical} &\url{https://github.com/wengong-jin/hgraph2graph}\\
MGM & Molecule generation & MPN & Nature Communications'21 &\cite{mahmood2021masked}  &\url{https://github.com/nyu-dl/ dl4chem-mgm66}\\
MoLeR &molecular generation &GNN &ICLR'22 &\cite{maziarz2022learning} & /\\
\midrule
VJTNN &molecular optimization &MPNN &ICLR'18 &\cite{jin2018learning} &\url{https://github.com/wengong-jin/iclr19-graph2graph}\\
MHG-VAE &Moleclar optimization &Hypergraph grammar VAE &ICML'19 &\cite{kajino2019molecular} &\url{https://github.com/ibm-research-tokyo/graph_grammar}\\
\midrule
AttSemiGAE & Adverse Drug-drug Interaction &Graph Auto Encoder &IJCAI'18 &\cite{ma2018drug} &\url{https://github.com/matenure/mvGAE}\\
E2E & Drug-target interaction &Graph CNN &IJCAI'18 &\cite{gao2018interpretable} &/ \\
KGNN &drug-drug interaction &GNN &IJCAI'20 &\cite{lin2020kgnn} &\url{https://github.com/xzenglab/KGNN} \\
SafeDrug & Drug-drug interaction & MPNN & IJCAI'21 &\cite{yangsafedrug} &\url{https://github.com/ycq091044/SafeDrug} \\
MDNN & Drug-drug interaction & GNN & IJCAI'21 &\cite{lyumdnn} &\url{https://github.com/YifanDengWHU/DDIMDL}\\
GemNet & Molecular interaction & MPNN & NeurIPS'21 &\cite{klicpera2021gemnet} &\url{https://www.in.tum.de/daml/gemnet/}\\
\midrule
ConfVAE &molecular conformation generation &GNN &ICML'21 &\cite{xu2021end} &\url{ https://github.com/MinkaiXu/ ConfVAE-ICML21}\\
\midrule
RationaleRL & Drug discovery & MPNN & PMLR'20 &\cite{jin2020multi} &\url{https://github.com/wengong-jin/multiobj-rationale}\\
\midrule
\midrule
\multicolumn{6}{c}{Sequence-based Learning} \\
\midrule
Seq2seq Fingerprint & Property prediction & Seq2seq & ACM-BCB'17 & \cite{xu2017seq2seq} &\url{https://github.com/XericZephyr/seq2seq-fingerprint}\\
Seq3seq Fingerprint & Property prediction & Seq2seq & ACM-BCB'18 & \cite{zhang2018seq3seq} & /\\
SMILES Transformer & Property prediction & Transformer &arxiv'19 & \cite{honda2019smiles} &\url{https://github.com/DSPsleeporg/smiles-transformer}\\
ChemBERTa & Property prediction & BERT &arxiv'20 & \cite{chithrananda2020chemberta} & /\\
MolBERT & Property prediction & BERT &NeurIPS workshop'20 &\cite{fabian2020molecular} &\url{https://ml4molecules.github.io} \\
\midrule
Found in Translation & Reaction prediction & Seq2seq & NeurIPS'17 &\cite{schwaller2018found} &\url{https://github.com/wengong-jin/nips17-rexgen} \\
Molecular Transformer & Reaction prediction & Transformer     & ACS Central Science'19 & \cite{schwaller2019molecular}  & \url{https://github.com/pschwllr/ MolecularTransformer}\\
\midrule
MDDRL & Molecular generation & RNN & Journal of Cheminformatics'17 &\cite{olivecrona2017molecular} &\url{ https://github.com/MarcusOlivecrona/REINVENT}\\
GEGL &molecular optimization &LSTM &NeurIPS'20 &\cite{ahn2020guiding}  &\url{ https://github.com/ sungsoo-ahn/genetic-expert-guided-learning}\\
UGMMT & Molecular optimization & VAE &KDD'21 &\cite{barshatski2021unpaired} &\url{https://github.com/guy-ba/UGMMT}\\
\midrule
Yield-BERT & Yield prediction & BERT & Machine learning: science and technology'21 & \cite{schwaller2021prediction} &\url{ https://rxn4chemistry.github.io/rxn_yields/} \\
\midrule
\midrule
\multicolumn{6}{c}{Fusion Learning} \\
\midrule
GraSeq & Property prediction & GraphSage+VAE & CIKM'20 &\cite{guo2020graseq} &\url{https://github.com/zhichunguo/GraSeq} \\
RetroXpert &retrosynthesis prediction &GAT+Seq2seq &NeurIPS'20 &\cite{yan2020retroxpert}  &\url{ https://github.com/uta-smile/RetroXpert}\\
MG-BERT & Property prediction & MPNN+BERT & briefings in bioinformatics'21 &\cite{zhang2021mg} & \url{https://github.com/zhang-xuan1314/Molecular-gra ph-BERT}\\
\bottomrule
\end{tabular}}}
\end{center}

\end{table*}


\comment{GGNN~\cite{li2016gated}}



==> tables/Papers_overview_old.tex <==
\begin{table*}
% \vspace{-0.15in}
\caption{Taxonomy and Representative Publications of Molecule Representation Learning.}
\vspace{-0.15in}
\label{tab:main_algorithm}
\begin{center}
\scale[0.6]{{\begin{tabular}{l|l|l|c|c|l|l|l}
\toprule
\textbf{Algorithm} & \textbf{Task} & \textbf{Encoder} &\textbf{Pretrain} &\textbf{Multi-task} &\textbf{Reference} &\textbf{Venue} &\textbf{Key Point}\\ 
\midrule \midrule
\multicolumn{8}{c}{Graph-based Learning} \\
\midrule
SAMPN & Property prediction & MPNN & $\times$ & $\times$ & \cite{tang2020self} & Journal of Cheminformatics'20 & Self-attention\\
AMPNN/EMNN  & Property prediction & MPNN & $\times$ & $\times$ & \cite{withnall2020building} & Journal of Cheminformatics'20 & Attention and edge memory schemes\\
GNN-FiLM & Property prediction & MPNN & $\times$ & $\times$ & \cite{brockschmidt2020gnn}& PCML'20 & Feature-wise module\\
MPNN & Property prediction & MPNN & $\times$ &  $\times$ &\cite{gilmer2017neural} & PMLR'17 & \\
PAR & Property prediction & GIN & $\surd$ & $\surd$ &\cite{wang2021property} & Neurips'21 & Property-aware relation networks\\
Pre-GNN & Property prediction & GIN & $\surd$ & $\times$ &\cite{hu2019strategies}& ICLR'20 & Pretraining GNN\\ Meta-MGNN & Property prediction & GIN & $\surd$ & $\surd$ & \cite{guo2021few}& WWW'21 & Few-shot setting\\
WLDN++ & Reaction prediction & GCN & $\times$ & $\times$ & \cite{coley2019graph}& Chemical Science' 19 & \\
WLDN & Reacton prediction & WLN & $\times$ & $\times$ & \cite{jin2017predicting}& NIPS'17 & \\
GTPN & Reaction prediction & MPNN & $\times$ & $\surd$ & \cite{do2019graph} & KDD'19 &  \\
MolR & Metric learning& GCN/GAT/SAGE/TAG & $\times$ & $\times$ & \cite{wang2021chemical}& ICLR'22 &\\
ELECTRO & Electron path prediction & GG-NN & $\times$ & $\times$ &\cite{bradshaw2018generative} & ICLR'19 & \\
MGM & Molecule generation & MPNN & $\times$ &  $\times$ &\cite{mahmood2021masked} & Nature Communications'21 &\\
JT-VAE & Molecule generation & MPNN & $\times$ & $\times$ &\cite{jin2018junction} & ICLR'18 & \\
\midrule
\midrule
\multicolumn{8}{c}{Sequence-based Learning} \\
\midrule
SA-BiLSTM & Property/toxicology/bioactivity & Bi-LSTM & $\times$ & $\times$ &\cite{zheng2019identifying} & Journal of Chemical Information and modeling'19 & \\
ChemBERTa & Property prediction & RoBERTa & $\surd$ & $\times$ & \cite{chithrananda2020chemberta}&arxiv'20 & \\
MolBERT & Property prediction & BERT & $\surd$ & $\times$ &\cite{fabian2020molecular} & arxiv'20 & \\
Seq2seq Fingerprint & Property prediction & Seq2seq & $\surd$ & $\times$ & \cite{xu2017seq2seq}& ACM-BCB'17 &\\
Seq3seq Fingerprint & Property prediction & Seq2seq & $\times$ & $\surd$ & \cite{zhang2018seq3seq}& ACM-BCB'18 & \\
SMILES Transformer & Property prediction & Transformer & $\surd$ & $\times$ & \cite{honda2019smiles} &arxiv'19 &\\
Molecular Transformer & Reaction prediction & Transformer & $\surd$ & $\times$ & \cite{schwaller2019molecular} & ACS Central Science'19 & \\
Found in Translation & Reaction prediction & Seq2seq & $\times$ & $\times$ &\cite{schwaller2018found} & NIPS'17 & Novel tokenize \\
MDDRL & Structure generation & RNN & $\times$ & $\surd$ &\cite{olivecrona2017molecular} & Journal of Cheminformatics'17 \\
Yield-BERT & Yield prediction & BERT & $\surd$ & $\times$ & \cite{schwaller2021prediction} & Machine learning: science and technology'21 & \\
\midrule
\midrule
\multicolumn{8}{c}{Fusion Learning} \\
\midrule
MG-BERT & Property prediction & MPNN+BERT & $\surd$ & $\times$ &\cite{zhang2021mg} & briefings in bioinformatics'21 & \\
GraSeq & Property prediction & GraphSage+VAE & $\times$ & $\surd$ &\cite{guo2020graseq} & CIKM'20 & \\
\bottomrule
\end{tabular}}}
\end{center}

\end{table*}

GG-NN\cite{li2015gated}, Weisfeiler-Lehman network\cite{}, GCN\cite{},

